Breaking the Million-Electron and 1 EFLOP/s Barriers: Biomolecular-Scale Ab Initio Molecular Dynamics Using MP2 Potentials

The accurate simulation of complex biochemical phenomena has historically been hampered by the computational requirements of high-fidelity molecular-modeling techniques. Quantum mechanical methods, such as ab initio wave-function (WF) theory, deliver the desired accuracy, but have impractical scaling for modelling biosystems with thousands of atoms. Combining molecular fragmentation with MP2 perturbation theory, this study presents an innovative approach that enables biomolecular-scale ab initio molecular dynamics (AIMD) simulations at WF theory level. Leveraging the resolution-of-the-identity approximation for Hartree-Fock and MP2 gradients, our approach eliminates computationally intensive four-center integrals and their gradients, while achieving near-peak performance on modern GPU architectures. The introduction of asynchronous time steps minimizes time step latency, overlapping computational phases and effectively mitigating load imbalances. Utilizing up to 9,400 nodes of Frontier and achieving 59% (1006.7 PFLOP/s) of its double-precision floating-point peak, our method enables us to break the million-electron and 1 EFLOP/s barriers for AIMD simulations with quantum accuracy.

==> jorges_past_writings.tex <==

The many flavours of AIMD have been actively developed and applied to a variety of problems over the last three decades. At its core, AIMD seeks to understand the time evolution of a chemical/physical system by obtaining the forces via \textit{ab initio} calculations such as Density Functional Theory (DFT), Hartree-Fock (HF), and post HF methods. However, \textit{ab initio} calculations are known to be computationally expensive ($\geq \mathcal{O}(N^3)$ ) and sometimes difficult to converge. The flavours of AIMD emerge from the approximations taken to obtain the forces and if the motion of the nuclei is coupled to the electronic motion. From the latter, there are adiabatic and non-adiabatic AIMD algorithms. Here, we will focus on adiabatic AIMD. 

The most prominent algorithms within adiabatic AIMD are namely: Born-Oppenheimer (BO), Car-Parinello (CP), Tight-Binding (TB), Path Integral (PI), and Quantum Monte Carlo (QMC). The most accurate and also the most computationally demanding one is BO-AIMD, since it relies on solving the electronic problem at every single time-step taken for the calculation. The rest of the methodologies, either reduce the number of times a full \textit{ab initio} calculations needs to be made (CP); or approximates the calculation with a cheaper, less computationally demanding method (PI, QMC). 

There is a delicate balance between the accuracy and computational expense of the method. In reality, it would be desirable to perform BO-AIMD on every system, since quantum effects are what give matter its properties. However, \textit{ab initio} calculations are limited by the size of the system they can target. Methods with predictive capabilities scale as $\geq \mathcal{O}(N^5)$ with respect to system size, making them impossible to apply to realistic size systems such as biomolecules and materials. 

The state-of-the-art in AIMD simulations can be divided into: novel methodologies to obtain the forces; and the use of high performance computing to accelerate simulations. 
